Polar Codes for CQ Channels: Decoding via Belief-Propagation with Quantum Messages

This paper considers the design and decoding of polar codes for general classical-quantum (CQ) channels. It focuses on decoding via belief-propagation with quantum messages (BPQM) and, in particular, the idea of paired-measurement BPQM (PM-BPQM) decoding. Since the PM-BPQM decoder admits a classical density evolution (DE) analysis, one can use DE to design a polar code for any CQ channel and then efficiently compute the trade-off between code rate and error probability. We have also implemented and tested a classical simulation of our PM-BPQM decoder for polar codes. While the decoder can be implemented efficiently on a quantum computer, simulating the decoder on a classical computer actually has exponential complexity. Thus, simulation results for the decoder are somewhat limited and are included primarily to validate our theoretical results.

==> tikz_preamble.tex <==

\tikzset
{
    vnodeStyle/.style =
    {
        % -- shape properties --
        circle,                                 % shape
%       rounded corners = 3mm,                  % kind of corner (and radius of the roundness)
%       minimum height  = 0.15\textwidth,       % | minimum size of the node
%       minimum width   = 0.9\textwidth,        % |
        minimum size    = 10pt,                %
        rotate          = 0,                    % angle of rotation
        scale           = 1.0,                  % scaling factor
        thick,                                  % thickness of the border
        %
        % -- colours properties --
        % filling: [ trasparent | monocolored | shaded]; decomment what you prefer
%       %                                       % transparent (all commented)
        fill            = bitcolor,             % monocolored
%       top color       = white,                % | filling of the node
%       bottom color    = red!50!black!20,      % |
        text            = black,                % colour of the fonts
        draw            = black,                % colour of the border
        %
        % -- fonts --
        font            = \scriptsize,              % shape of the font (or dimension, like \tiny)
%       text centered,                          % text alignment [text centered | text badly centered | text justified | text ragged | text badly ragged]
        inner xsep      = 0mm,                  % minimum distance between text and borders along x dimension
        inner ysep      = 0mm,                  % minimum distance between text and borders along y dimension
        text height     = 0.2cm,
        text depth      = 0.12cm,
    }
}






\tikzset
{
    cnodeStyle/.style =
    {
        % -- shape properties --
        rectangle,                                  % shape
%        rounded corners = 1mm,                  % kind of corner (and radius of the roundness)
%       minimum height  = 0.15\textwidth,       % | minimum size of the node
%       minimum width   = 0.9\textwidth,        % |
        minimum size    = 8pt,                %
        rotate          = 0,                    % angle of rotation
        scale           = 1.0,                  % scaling factor
        thick,                                  % thickness of the border
        %
        % -- colours properties --
        % filling: [ trasparent | monocolored | shaded]; decomment what you prefer
%       %                                       % transparent (all commented)
        fill            = checkcolor,           % monocolored
%       top color       = white,                % | filling of the node
%       bottom color    = red!50!black!20,      % |
        text            = black,                % colour of the fonts
        draw            = black,                % colour of the border
        %
        % -- fonts --
        font            = \scriptsize,              % shape of the font (or dimension, like \tiny)
        text centered,                          % text alignment [text centered | text badly centered | text justified | text ragged | text badly ragged]
%       text height     = 1mm,                  % ! minimum size of the text    % NOT WORKING
%       text depth      = 1mm,                  % !
        inner xsep      = 0mm,                  % minimum distance between text and borders along x dimension
        inner ysep      = 0mm                   % minimum distance between text and borders along y dimension
    }
}




\tikzset {
    WarningTextStyle/.style =
    {
        rectangle,                      % shape
        rounded corners = 0.6cm,        %
        minimum size    = 1.2cm,          %
        rotate          = 0,            % angle of rotation
        scale           = 1.0,          % scaling factor
        thick,                          % thickness of the border
        fill            = red!10,       % monocolored
        text            = red!10!black, % colour of the fonts
        draw            = red,          % colour of the border
        font            = \large,       % shape of the font (or dimension, like \tiny)
        text centered,                  % text alignment
        text width      = 10cm,         % text alignment
        inner xsep      = 0.1cm,        % minimum distance between text and borders along x dimension
        inner ysep      = 0.1cm         % minimum distance between text and borders along y dimension
    }
}



\tikzset {
    RemarkTextStyle/.style =
    {
        rectangle,                      % shape
        rounded corners = 0.6cm,        %
        minimum size    = 1.2cm,          %
        rotate          = 0,            % angle of rotation
        scale           = 1.0,          % scaling factor
        thick,                          % thickness of the border
        fill            = blue!10,       % monocolored
        text            = blue!10!black, % colour of the fonts
        draw            = blue,          % colour of the border
        font            = \large,       % shape of the font (or dimension, like \tiny)
        text centered,                  % text alignment
        text width      = 10cm,         % text alignment
        inner xsep      = 0.3cm,        % minimum distance between text and borders along x dimension
        inner ysep      = 0.3cm         % minimum distance between text and borders along y dimension
    }
}




\tikzset
{
    FittingStyle/.style =
    {
        % -- shape properties --
        shape = ellipse,                            % shape
%       rounded corners = 1mm,                  % kind of corner (and radius of the roundness)
%       minimum height  = 0.15\textwidth,       % | minimum size of the node
%       minimum width   = 0.9\textwidth,        % |
%       minimum size    = 4.5mm,                %
%       rotate          = 0,                    % angle of rotation
        scale           = 1.0,                  % scaling factor
        thick,                                  % thickness of the border
        %
        % -- colours properties --
        % filling: [ trasparent | monocolored | shaded]; decomment what you prefer
%       %                                       % transparent (all commented)
%       fill            = black!30,             % monocolored
%       top color       = white,                % | filling of the node
%       bottom color    = red!50!black!20,      % |
%       text            = black,                % colour of the fonts
        draw            = red,              % colour of the border
        %
        % -- fonts --
%       font            = \scriptsize,              % shape of the font (or dimension, like \tiny)
%       text centered,                          % text alignment [text centered | text badly centered | text justified | text ragged | text badly ragged]
%       text height     = 1mm,                  % ! minimum size of the text    % NOT WORKING
%       text depth      = 1mm,                  % !
        inner xsep      = 0mm,                  % minimum distance between text and borders along x dimension
        inner ysep      = 0mm                   % minimum distance between text and borders along y dimension
    }
}



\tikzset
{
    GenericNodeStyle/.style =
    {
        % -- shape properties --
        shape = rectangle,                          % shape
        rounded corners = 3mm,                  % kind of corner (and radius of the roundness)
        minimum height  = 1cm,                  % | minimum size of the node
        minimum width   = 2cm,                  % |
        scale           = 1.0,                  % scaling factor
        thick,                                  % thickness of the border
        %
        % -- colours properties --
        % filling: [ trasparent | monocolored | shaded]; decomment what you prefer
%       %                                       % transparent (all commented)
        fill            = green!10!white,               % monocolored
%       top color       = white,                % | filling of the node
%       bottom color    = red!50!black!20,      % |
%       text            = black,                % colour of the fonts
        draw            = green,                % colour of the border
        %
        % -- fonts --
%       font            = \scriptsize,              % shape of the font (or dimension, like \tiny)
%       text centered,                          % text alignment [text centered | text badly centered | text justified | text ragged | text badly ragged]
%       text height     = 1mm,                  % ! minimum size of the text    % NOT WORKING
%       text depth      = 1mm,                  % !
        inner xsep      = 3mm,                  % minimum distance between text and borders along x dimension
        inner ysep      = 3mm                   % minimum distance between text and borders along y dimension
    }
}




\tikzset
{
    NormalNodeStyle/.style =
    {
        shape = circle,                         % shape
        minimum size    = 20,                   %
        rotate          = 0,                    % angle of rotation
        scale           = 1.0,                  % scaling factor
        thick,                                  % thickness of the border
        text            = black,                % colour of the fonts
        draw            = black,                % colour of the border
        font            = \small,               % shape of the font (or dimension, like \tiny)
        text centered,                          % text alignment
        inner xsep      = 0,                    % minimum distance between text and borders along x dimension
        inner ysep      = 0                     % minimum distance between text and borders along y dimension
    }
}



\tikzset
{
    BridgeNodeStyle/.style =
    {
        circle,                                 % shape
        minimum size    = 20,                   %
        rotate          = 0,                    % angle of rotation
        scale           = 1.0,                  % scaling factor
        thick,                                  % thickness of the border
        fill            = black!30,             % monocolored
        text            = black,                % colour of the fonts
        draw            = black,                % colour of the border
        font            = \small,               % shape of the font (or dimension, like \tiny)
        text centered,                          % text alignment
        inner xsep      = 0,                    % minimum distance between text and borders along x dimension
        inner ysep      = 0                     % minimum distance between text and borders along y dimension
    }
}






\tikzstyle{sNormalBlockStyle} = [
    draw,
    rectangle,
    rounded corners = 0.1cm,
    fill            = blue!20,
    minimum height  = 3em,
    minimum width   = 6em,
]





\tikzstyle{sSumBlockStyle} =
[
    shape           = circle,
    draw,
    fill            = blue!20,
]




\tikzstyle{sArrowsStyle} =
[
    thick,
    color   = black,
    -latex
]




\tikzstyle{sLinesStyle} =
[
    thick,
    color   = black,
    -
]




\tikzstyle{sTextBlockStyle} =
[
    draw,
    rectangle,
    drop shadow,
    rounded corners = 0.1cm,
    fill            = blue!10,
    thick,
    inner xsep      = 0.2cm,        % minimum distance between text and borders along x dimension
    inner ysep      = 0.2cm         % minimum distance between text and borders along y dimension
]



\tikzfading % DO NOT CHANGE THE ORDER OF THE COLORS otherwise it will not work
[
    name            = middle,
    top color       = transparent!100,
    bottom color    = transparent!100,
    middle color    = transparent!00,
]



\tikzstyle{sCoalFiredPlant} =
[
    shape           = rectangle,
    minimum height  = 0.5cm,
    minimum width   = 0.5cm,
    rounded corners = 0.1cm,
    fill            = black!20,
    draw            = black,
    line width      = 0.1cm,
    inner xsep      = 0.2cm,
    inner ysep      = 0.2cm
]

